Dark Energy Survey Year 3 Results: Clustering Redshifts -- Calibration of the Weak Lensing Source Redshift Distributions with redMaGiC and BOSS/eBOSS

We present the calibration of the Dark Energy Survey Year 3 (DES Y3) weak lensing source galaxy redshift distributions $n(z)$ from clustering measurements. In particular, we cross-correlate the weak lensing (WL) source galaxies sample with redMaGiC galaxies (luminous red galaxies with secure photometric redshifts) and a spectroscopic sample from BOSS/eBOSS to estimate the redshift distribution of the DES sources sample. Two distinct methods for using the clustering statistics are described. The first uses the clustering information independently to estimate the mean redshift of the source galaxies within a redshift window, as done in the DES Y1 analysis. The second method establishes a likelihood of the clustering data as a function of $n(z)$, which can be incorporated into schemes for generating samples of $n(z)$ subject to combined clustering and photometric constraints. Both methods incorporate marginalisation over various astrophysical systematics, including magnification and redshift-dependent galaxy-matter bias. We characterise the uncertainties of the methods in simulations; the first method recovers the mean $z$ of tomographic bins to RMS (precision) of $\sim 0.014$. Use of the second method is shown to vastly improve the accuracy of the shape of $n(z)$ derived from photometric data. The two methods are then applied to the DES Y3 data.

==> Y1_analysis.tex <==
\section{Y1 re-analysis}

\begin{itemize}
    \item should add a plot comparing BPZ distributions, WZ y1 (using higher lum sample) and WZ obtained with the new method (high density sample, + theory + bias corrections)
    \item should add a table with all the shifts for all the possible types of runs
    \item write what you did, and what changes wrt y1
\end{itemize}

We (partially) test here the new method presented in \S~\ref{sect:methodology} applying it on DES Y1 data. In the DES Y1 analysis, as previously mentioned, the galaxy-matter biases and clustering of dark matter were not modelled and were assumed as constant in each photo-z bin. As a consequence, the DES Y1 clustering-$z$ systematic error budget had to account for these erroneous assumptions. We tested whether by measuring these parameters we would obtain values compatible with the Y1 results within systematic uncertainties. In this test the ``Y3 method'' includes the modelling for $b_{\rm r}$ and $w_{\rm DM}$. 

For consistency with the DES Y1 results presented in  \cite{Davis2017aaa}, we used that same binning scheme, dividing the \redmagic\ sample into 50 bins in the redshift range [0, 1].
Magnification effects were not included as systematic uncertainties in this test like for Y1, since restricting to two sigma the window over which the mean is computed eliminates the tails, where magnification effects give their largest contribution.  
In Y1 the systematics introduced by $b_u$, $b_r$ and $w_{DM}$ were considered as one single bias. In Y3 these have been examined separately: only the $b_u$ enters into play as a systematic effect, whether the $b_r$ and $w_{DM}$ have been modelled and therefore do not contribute anymore to the error budget. 

(Test performed in simulation has suggested that the br and wdm might give opposite contribution, but relying solely on simulation to estimate a correlation between these two quantities seems a stretch.) 


In Figure \ref{fig:y1y3distr} the distribution corresponding to the two methods are reported, for each tomographic bin. As shown in Figure \ref{fig:y1y3shifts}, the shifts over the mean recovered with the Y3 method are well compatible with the Y1 estimates. 


\begin{figure*}
    \begin{center}
    \includegraphics[width=0.8 \textwidth]{figures/y1y3distr.png}
    \caption{Estimated redshift distribution on Y1 data for each tomographic bin, using two different methods: Y1 method and Y3 method, where the br and wdm were modelled.}\label{fig:y1y3distr}
    \end{center}
    
\end{figure*}

\begin{figure*}
    \begin{center}
    \includegraphics[width=0.9 \textwidth]{figures/y1y3shifts.png}
    \caption{Estimated shifts on Y1 data for each tomographic bin, using two different methods: Y1 method and Y3 method, where the br and wdm were modelled.}\label{fig:y1y3shifts}
    \end{center}
    
\end{figure*}

==> authors_MNRAS.tex <==
%MNRAS
\author[Authors]{
\parbox{\textwidth}{
\Large 
Authors
}
}
\vspace{0.2cm}








==> summary_tests_sims.tex <==
\subsection{Summary tests on simulations}\label{summary1}

\gnote{I think it might be better to merge this section with the discussion/conclusions at the end of the paper.}

In the previous subsections we discussed two different methods to inform the posterior of a photo-$z$ code (SOMPZ) with clustering information: the ``mean-matching'' and ``full-shape'' methods. The former is similar in spirit to what has been implemented in the DES Y1 analysis \citep{Gatti2018,Davis2018}, and it is mostly able to calibrate the mean of the SOMPZ N(z); the second is a novel method that allows to use to also inform the shape of the SOMPZ N(z). 

Both methods have not proven to be particularly useful tightening the mean of the SOMPZ N(z) realisations. This is mostly due to the superior constraining power of the SOMPZ method: the typical constraining power of the clustering methods on the mean of the redshift distribution (in an interval excluding the tails of the distributions) is $\sim 0.015$, whereas the SOMPZ uncertainties are much smaller (see Table~\ref{tableres} or the plots in Appendix~\ref{sect:Appendix_marg}). A caveat here is that the SOMPZ uncertainties in simulations do not fully capture uncertainties and biases in the spectroscopic samples used for the SOMPZ method in data, or photometric calibration biases (which are added at a later stage). We tested, however, that even in the case where the simulated SOMPZ uncertainties were as twice as large, the clustering redshift methods would not be able to tighten the SOMPZ constrains on the mean. 

Despite not being able to tighten the constraints on the mean of the SOMPZ realisations, the shape-matching method is able to tighten the SOMPZ scatter. This is mostly a consequence of the complementarity of the SOMPZ and clustering constraints, the former being mostly driven by sample variance, the latter being limited by slowly-varying (in terms of redshift evolution) systematics. For this reason, the full-shape method is the standard method chosen in the DES Y3 analysis, and the mean-matching method is only used as crosscheck.

In literature there exist other methods to calibrate the posterior of photo-$z$ codes using the clustering information (e.g., \citealt{Choi2016,Davis2017aaa,vandenBusch2020}). In general, these works calibrate the photo-$z$ posterior through a coherent redshift ``shift'', while trying to minimise a $\chi^2$ between the clustering $N(z)$ and the photo-$z$ posterior. These approaches can lead to biased results if the shape of the photo-$z$ posterior differs from the truth, or if clustering  systematics are not taken into account by a sufficiently flexible model, as noted by \cite{Gatti2018,vandenBusch2020}. In this respect, our implementation of the full-shape method should be robust against these sort of bias, as we are properly accounting for uncertainties in the shapes of both clustering and SOMPZ estimates.

